Not All Unlabeled Data are Equal: Learning to Weight Data in Semi-supervised Learning

Existing semi-supervised learning (SSL) algorithms use a single weight to balance the loss of labeled and unlabeled examples, i.e., all unlabeled examples are equally weighted. But not all unlabeled data are equal. In this paper we study how to use a different weight for every unlabeled example. Manual tuning of all those weights -- as done in prior work -- is no longer possible. Instead, we adjust those weights via an algorithm based on the influence function, a measure of a model's dependency on one training example. To make the approach efficient, we propose a fast and effective approximation of the influence function. We demonstrate that this technique outperforms state-of-the-art methods on semi-supervised image and language classification tasks.

==> alb_four_figure.tex <==
%!TEX root = main.tex
\begin{figure}[t]
\vsp{-0.5cm}
\includegraphics[width=0.245\textwidth]{fig/analysis/abl-one-lambda.pdf}
\includegraphics[width=0.245\textwidth]{fig/analysis/abl-adam.pdf}
\includegraphics[width=0.245\textwidth]{fig/analysis/abl-val-size.pdf}
\includegraphics[width=0.245\textwidth]{fig/analysis/abl-hess.pdf}
\vsp{-0.5cm}
\caption{
\textbf{1st fig:} Test error comparison between tuning a single weight and per-example weights across different amounts of labeled data. \textbf{2nd fig:} Validation error during training of models using different optimizers. \textbf{3th fig:} Test error comparisons across models using different validation set sizes. All experiments are conducted on CIFAR-10. \textbf{4th fig:} Validation error rate (\%) over training time comparisons between different approximations of influence function.
}
\label{fig:abl-three}
\vsp{-0.5cm}
\end{figure}

==> stl_results.tex <==
%!TEX root = main.tex
\begin{table}[t]
\resizebox{\columnwidth}{!}{
\centering
\begin{tabular}{c | c c | c c}
\specialrule{.15em}{.05em}{.05em} 
 & & &  \multicolumn{2}{|c}{\# Labeled }\\
Methods & Model & \# Param. & 1000 & 5000  \\
\hline
CutOut & WRN-16-8 & 11M &-  & 12.74$\pm$0.23 \\
IIC  & RN-34 & 21.3M & -  & 11.20 \\
SWWAE & VGG & 132M & 25.70 &- \\
CC-GAN2 & VGG & 132M & 22.20 &- \\
MixMatch & WRN-37-2 &23.8M  &  10.18$\pm$1.46 & 5.59 \\
UDA & WRN-37-2 & 23.8M & 7.66$\pm$0.56 &-\\
Re-MixMatch & WRN-37-2 & 23.8M & 6.18$\pm$1.24 &-\\
\hline
Ours & WRN-37-2 & 23.8M &  \\
\specialrule{.15em}{.05em}{.05em} 
\end{tabular}}
\caption{STL-10 error rate (\%) using 1000-label splits or the entire 5000-label training set. We compare to recent publications including CutOut~\citep{devries2017cutout}, IIC~\citep{ji2019iic}, SWWAE~\citep{zhao2015stacked}, CC-GAN2~\citep{DentonGF16}, MixMatch~\citep{berthelot2019mixmatch}, UDA~\citep{xie2019uda}, and Re-MixMatch~\citep{berthelot2020remixmatch}. (RN: ResNet, WRN: Wide ResNet.) For our method, we report the mean and standard deviation over 5 runs.}
\label{tab:res-stl}
\vspace{-2em}
\end{table}
